Detection of two TeV gamma-ray outbursts from NGC 1275 by LHAASO

The Water Cherenkov Detector Array (WCDA) is one of the components of Large High Altitude Air Shower Observatory (LHAASO) and can monitor any sources over two-thirds of the sky for up to 7 hours per day with >98\% duty cycle. In this work, we report the detection of two outbursts of the Fanaroff-Riley I radio galaxy NGC 1275 that were detected by LHAASO-WCDA between November 2022 and January 2023 with statistical significance of 5.2~$\sigma$ and 8.3~$\sigma$. The observed spectral energy distribution in the range from 500 GeV to 3 TeV is fitted by a power-law with a best-fit spectral index of $\alpha=-3.37\pm0.52$ and $-3.35\pm0.29$, respectively. The outburst flux above 0.5~TeV was ($4.55\pm 4.21)\times~10^{-11}~\rm cm^{-2}~s^{-1}$ and ($3.45\pm 1.78)\times~10^{-11}~\rm cm^{-2}~s^{-1}$, corresponding to 60\%, 45\% of Crab Nebula flux. Variation analysis reveals the variability time-scale of days at the TeV energy band. A simple test by one-zone synchrotron self-Compton model reproduces the data in the gamma-ray band well.

==> Detection_of_two_TeV_gamma-ray_outbursts_from_NGC_1275_by_LHAASO/Science20240601.tex <==
Zhen Cao$^{1,2,3}$,
F. Aharonian$^{4,5}$,
Axikegu$^{6}$,
Y.X. Bai$^{1,3}$,
Y.W. Bao$^{7}$,
D. Bastieri$^{8}$,
X.J. Bi$^{1,2,3}$,
Y.J. Bi$^{1,3}$,
W. Bian$^{9}$,
A.V. Bukevich$^{10}$,
Q. Cao$^{11}$,
W.Y. Cao$^{12}$,
Zhe Cao$^{13,12}$,
J. Chang$^{14}$,
J.F. Chang$^{1,3,13}$,
A.M. Chen$^{9}$,
E.S. Chen$^{1,2,3}$,
H.X. Chen$^{15}$,
Liang Chen$^{16}$,
Lin Chen$^{6}$,
Long Chen$^{6}$,
M.J. Chen$^{1,3}$,
M.L. Chen$^{1,3,13}$,
Q.H. Chen$^{6}$,
S. Chen$^{17}$,
S.H. Chen$^{1,2,3}$,
S.Z. Chen$^{1,3}$,
T.L. Chen$^{18}$,
Y. Chen$^{7}$,
N. Cheng$^{1,3}$,
Y.D. Cheng$^{1,2,3}$,
M.C. Chu$^{19}$,
M.Y. Cui$^{14}$,
S.W. Cui$^{11}$,
X.H. Cui$^{20}$,
Y.D. Cui$^{21}$,
B.Z. Dai$^{17}$,
H.L. Dai$^{1,3,13}$,
Z.G. Dai$^{12}$,
Danzengluobu$^{18}$,
X.Q. Dong$^{1,2,3}$,
K.K. Duan$^{14}$,
J.H. Fan$^{8}$,
Y.Z. Fan$^{14}$,
J. Fang$^{17}$,
J.H. Fang$^{15}$,
K. Fang$^{1,3}$,
C.F. Feng$^{22}$,
H. Feng$^{1}$,
L. Feng$^{14}$,
S.H. Feng$^{1,3}$,
X.T. Feng$^{22}$,
Y. Feng$^{15}$,
Y.L. Feng$^{18}$,
S. Gabici$^{23}$,
B. Gao$^{1,3}$,
C.D. Gao$^{22}$,
Q. Gao$^{18}$,
W. Gao$^{1,3}$,
W.K. Gao$^{1,2,3}$,
M.M. Ge$^{17}$,
T.T. Ge$^{21}$,
L.S. Geng$^{1,3}$,
G. Giacinti$^{9}$,
G.H. Gong$^{24}$,
Q.B. Gou$^{1,3}$,
M.H. Gu$^{1,3,13}$,
F.L. Guo$^{16}$,
J. Guo$^{24}$,
X.L. Guo$^{6}$,
Y.Q. Guo$^{1,3}$,
Y.Y. Guo$^{14}$,
Y.A. Han$^{25}$,
O.A. Hannuksela$^{19}$,
M. Hasan$^{1,2,3}$,
H.H. He$^{1,2,3}$,
H.N. He$^{14}$,
J.Y. He$^{14}$,
Y. He$^{6}$,
Y.K. Hor$^{21}$,
B.W. Hou$^{1,2,3}$,
C. Hou$^{1,3}$,
X. Hou$^{26}$,
H.B. Hu$^{1,2,3}$,
Q. Hu$^{12,14}$,
S.C. Hu$^{1,3,27}$,
C. Huang$^{7}$,
D.H. Huang$^{6}$,
T.Q. Huang$^{1,3}$,
W.J. Huang$^{21}$,
X.T. Huang$^{22}$,
X.Y. Huang$^{14}$,
Y. Huang$^{1,2,3}$,
Y.Y. Huang$^{7}$,
X.L. Ji$^{1,3,13}$,
H.Y. Jia$^{6}$,
K. Jia$^{22}$,
H.B. Jiang$^{1,3}$,
K. Jiang$^{13,12}$,
X.W. Jiang$^{1,3}$,
Z.J. Jiang$^{17}$,
M. Jin$^{6}$,
M.M. Kang$^{28}$,
I. Karpikov$^{10}$,
D. Khangulyan$^{1,3}$,
D. Kuleshov$^{10}$,
K. Kurinov$^{10}$,
B.B. Li$^{11}$,
C.M. Li$^{7}$,
Cheng Li$^{13,12}$,
Cong Li$^{1,3}$,
D. Li$^{1,2,3}$,
F. Li$^{1,3,13}$,
H.B. Li$^{1,3}$,
H.C. Li$^{1,3}$,
Jian Li$^{12}$,
Jie Li$^{1,3,13}$,
K. Li$^{1,3}$,
S.D. Li$^{16,2}$,
W.L. Li$^{22}$,
W.L. Li$^{9}$,
X.R. Li$^{1,3}$,
Xin Li$^{13,12}$,
Y.Z. Li$^{1,2,3}$,
Zhe Li$^{1,3}$,
Zhuo Li$^{29}$,
E.W. Liang$^{30}$,
Y.F. Liang$^{30}$,
S.J. Lin$^{21}$,
B. Liu$^{12}$,
C. Liu$^{1,3}$,
D. Liu$^{22}$,
D.B. Liu$^{9}$,
H. Liu$^{6}$,
H.D. Liu$^{25}$,
J. Liu$^{1,3}$,
J.L. Liu$^{1,3}$,
M.Y. Liu$^{18}$,
R.Y. Liu$^{7}$,
S.M. Liu$^{6}$,
W. Liu$^{1,3}$,
Y. Liu$^{8}$,
Y.N. Liu$^{24}$,
Q. Luo$^{21}$,
Y. Luo$^{9}$,
H.K. Lv$^{1,3}$,
B.Q. Ma$^{29}$,
L.L. Ma$^{1,3}$,
X.H. Ma$^{1,3}$,
J.R. Mao$^{26}$,
Z. Min$^{1,3}$,
W. Mitthumsiri$^{31}$,
H.J. Mu$^{25}$,
Y.C. Nan$^{1,3}$,
A. Neronov$^{23}$,
K.C.Y. Ng$^{19}$,
L.J. Ou$^{8}$,
P. Pattarakijwanich$^{31}$,
Z.Y. Pei$^{8}$,
J.C. Qi$^{1,2,3}$,
M.Y. Qi$^{1,3}$,
B.Q. Qiao$^{1,3}$,
J.J. Qin$^{12}$,
A. Raza$^{1,2,3}$,
D. Ruffolo$^{31}$,
A. S\'aiz$^{31}$,
M. Saeed$^{1,2,3}$,
D. Semikoz$^{23}$,
L. Shao$^{11}$,
O. Shchegolev$^{10,32}$,
X.D. Sheng$^{1,3}$,
F.W. Shu$^{33}$,
H.C. Song$^{29}$,
Yu.V. Stenkin$^{10,32}$,
V. Stepanov$^{10}$,
Y. Su$^{14}$,
D.X. Sun$^{12,14}$,
Q.N. Sun$^{6}$,
X.N. Sun$^{30}$,
Z.B. Sun$^{34}$,
J. Takata$^{35}$,
P.H.T. Tam$^{21}$,
Q.W. Tang$^{33}$,
R. Tang$^{9}$,
Z.B. Tang$^{13,12}$,
W.W. Tian$^{2,20}$,
L.H. Wan$^{21}$,
C. Wang$^{34}$,
C.B. Wang$^{6}$,
G.W. Wang$^{12}$,
H.G. Wang$^{8}$,
H.H. Wang$^{21}$,
J.C. Wang$^{26}$,
Kai Wang$^{7}$,
Kai Wang$^{35}$,
L.P. Wang$^{1,2,3}$,
L.Y. Wang$^{1,3}$,
P.H. Wang$^{6}$,
R. Wang$^{22}$,
W. Wang$^{21}$,
X.G. Wang$^{30}$,
X.Y. Wang$^{7}$,
Y. Wang$^{6}$,
Y.D. Wang$^{1,3}$,
Y.J. Wang$^{1,3}$,
Z.H. Wang$^{28}$,
Z.X. Wang$^{17}$,
Zhen Wang$^{9}$,
Zheng Wang$^{1,3,13}$,
D.M. Wei$^{14}$,
J.J. Wei$^{14}$,
Y.J. Wei$^{1,2,3}$,
T. Wen$^{17}$,
C.Y. Wu$^{1,3}$,
H.R. Wu$^{1,3}$,
Q.W. Wu$^{35}$,
S. Wu$^{1,3}$,
X.F. Wu$^{14}$,
Y.S. Wu$^{12}$,
S.Q. Xi$^{1,3}$,
J. Xia$^{12,14}$,
G.M. Xiang$^{16,2}$,
D.X. Xiao$^{11}$,
G. Xiao$^{1,3}$,
Y.L. Xin$^{6}$,
Y. Xing$^{16}$,
D.R. Xiong$^{26}$,
Z. Xiong$^{1,2,3}$,
D.L. Xu$^{9}$,
R.F. Xu$^{1,2,3}$,
R.X. Xu$^{29}$,
W.L. Xu$^{28}$,
L. Xue$^{22}$,
D.H. Yan$^{17}$,
J.Z. Yan$^{14}$,
T. Yan$^{1,3}$,
C.W. Yang$^{28}$,
C.Y. Yang$^{26}$,
F. Yang$^{11}$,
F.F. Yang$^{1,3,13}$,
L.L. Yang$^{21}$,
M.J. Yang$^{1,3}$,
R.Z. Yang$^{12}$,
W.X. Yang$^{8}$,
Y.H. Yao$^{1,3}$,
Z.G. Yao$^{1,3}$,
L.Q. Yin$^{1,3}$,
N. Yin$^{22}$,
X.H. You$^{1,3}$,
Z.Y. You$^{1,3}$,
Y.H. Yu$^{12}$,
Q. Yuan$^{14}$,
H. Yue$^{1,2,3}$,
H.D. Zeng$^{14}$,
T.X. Zeng$^{1,3,13}$,
W. Zeng$^{17}$,
M. Zha$^{1,3}$,
B.B. Zhang$^{7}$,
F. Zhang$^{6}$,
H. Zhang$^{9}$,
H.M. Zhang$^{7}$,
H.Y. Zhang$^{17}$,
J.L. Zhang$^{20}$,
Li Zhang$^{17}$,
P.F. Zhang$^{17}$,
P.P. Zhang$^{12,14}$,
R. Zhang$^{14}$,
S.B. Zhang$^{2,20}$,
S.R. Zhang$^{11}$,
S.S. Zhang$^{1,3}$,
X. Zhang$^{7}$,
X.P. Zhang$^{1,3}$,
Y.F. Zhang$^{6}$,
Yi Zhang$^{1,14}$,
Yong Zhang$^{1,3}$,
B. Zhao$^{6}$,
J. Zhao$^{1,3}$,
L. Zhao$^{13,12}$,
L.Z. Zhao$^{11}$,
S.P. Zhao$^{14}$,
X.H. Zhao$^{26}$,
F. Zheng$^{34}$,
W.J. Zhong$^{7}$,
B. Zhou$^{1,3}$,
H. Zhou$^{9}$,
J.N. Zhou$^{16}$,
M. Zhou$^{33}$,
P. Zhou$^{7}$,
R. Zhou$^{28}$,
X.X. Zhou$^{1,2,3}$,
X.X. Zhou$^{6}$,
B.Y. Zhu$^{12,14}$,
C.G. Zhu$^{22}$,
F.R. Zhu$^{6}$,
H. Zhu$^{20}$,
K.J. Zhu$^{1,2,3,13}$,
Y.C. Zou$^{35}$,
X. Zuo$^{1,3}$,
(The LHAASO Collaboration)
$^{1}$ Key Laboratory of Particle Astrophysics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ TIANFU Cosmic Ray Research Center, Chengdu, Sichuan,  China\\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{6}$ School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China\\
$^{7}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{8}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{9}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{10}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia\\
$^{11}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{12}$ University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{13}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{14}$ Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{15}$ Research Center for Astronomical Computing, Zhejiang Laboratory, 311121 Hangzhou, Zhejiang, China\\
$^{16}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{17}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{18}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{19}$ Department of Physics, The Chinese University of Hong Kong, Shatin, New Territories, Hong Kong, China\\
$^{20}$ Key Laboratory of Radio Astronomy and Technology, National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{21}$ School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China\\
$^{22}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{23}$ APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France\\
$^{24}$ Department of Engineering Physics \& Department of Astronomy, Tsinghua University, 100084 Beijing, China\\
$^{25}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{26}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{27}$ China Center of Advanced Science and Technology, Beijing 100190, China\\
$^{28}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{29}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{30}$ Guangxi Key Laboratory for Relativistic Astrophysics, School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{31}$ Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand\\
$^{32}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{33}$ Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology, Nanchang University, 330031 Nanchang, Jiangxi, China\\
$^{34}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
$^{35}$ School of Physics, Huazhong University of Science and Technology, Wuhan 430074, Hubei, China\\


==> Detection_of_two_TeV_gamma-ray_outbursts_from_NGC_1275_by_LHAASO/affi.tex <==
\twocolumn

\vspace*{0.5cm}
\noindent $^{1}$ Key Laboratory of Particle Astrophysics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ TIANFU Cosmic Ray Research Center, Chengdu, Sichuan,  China\\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{6}$ School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China\\
$^{7}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{8}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{9}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{10}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia\\
$^{11}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{12}$ University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{13}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{14}$ Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{15}$ Research Center for Astronomical Computing, Zhejiang Laboratory, 311121 Hangzhou, Zhejiang, China\\
$^{16}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{17}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{18}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{19}$ Department of Physics, The Chinese University of Hong Kong, Shatin, New Territories, Hong Kong, China\\
$^{20}$ Key Laboratory of Radio Astronomy and Technology, National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{21}$ School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China\\
$^{22}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{23}$ APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France\\
$^{24}$ Department of Engineering Physics \& Department of Astronomy, Tsinghua University, 100084 Beijing, China\\
$^{25}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{26}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{27}$ China Center of Advanced Science and Technology, Beijing 100190, China\\
$^{28}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{29}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{30}$ Guangxi Key Laboratory for Relativistic Astrophysics, School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{31}$ Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand\\
$^{32}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{33}$ Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology, Nanchang University, 330031 Nanchang, Jiangxi, China\\
$^{34}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
$^{35}$ School of Physics, Huazhong University of Science and Technology, Wuhan 430074, Hubei, China\\

==> Detection_of_two_TeV_gamma-ray_outbursts_from_NGC_1275_by_LHAASO/name.tex <==
\author[LHAASO Collaboration]{\parbox{\textwidth}{
\normalsize
%name.tex
%\parbox{\textwidth}{
%\normalsize
Zhen Cao$^{1,2,3}$,
F. Aharonian$^{4,5}$,
Axikegu$^{6}$,
Y.X. Bai$^{1,3}$,
Y.W. Bao$^{7}$,
D. Bastieri$^{8}$,
X.J. Bi$^{1,2,3}$,
Y.J. Bi$^{1,3}$,
W. Bian$^{9}$,
A.V. Bukevich$^{10}$,
Q. Cao$^{11}$,
W.Y. Cao$^{12}$,
Zhe Cao$^{13,12}$,
J. Chang$^{14}$,
J.F. Chang$^{1,3,13}$,
A.M. Chen$^{9}$,
E.S. Chen$^{1,2,3}$,
H.X. Chen$^{15}$,
Liang Chen$^{16}$,
Lin Chen$^{6}$,
Long Chen$^{6}$,
M.J. Chen$^{1,3}$,
M.L. Chen$^{1,3,13}$,
Q.H. Chen$^{6}$,
S. Chen$^{17}$,
S.H. Chen$^{1,2,3}$,
S.Z. Chen$^{1,3}$,
T.L. Chen$^{18}$,
Y. Chen$^{7}$,
N. Cheng$^{1,3}$,
Y.D. Cheng$^{1,2,3}$,
M.C. Chu$^{19}$,
M.Y. Cui$^{14}$,
S.W. Cui$^{11}$,
X.H. Cui$^{20}$,
Y.D. Cui$^{21}$,
B.Z. Dai$^{17}$,
H.L. Dai$^{1,3,13}$,
Z.G. Dai$^{12}$,
Danzengluobu$^{18}$,
X.Q. Dong$^{1,2,3}$,
K.K. Duan$^{14}$,
J.H. Fan$^{8}$,
Y.Z. Fan$^{14}$,
J. Fang$^{17}$,
J.H. Fang$^{15}$,
K. Fang$^{1,3}$,
C.F. Feng$^{22}$\thanks{\href{mailto: fengcf@sdu.edu.cn}{fengcf@sdu.edu.cn}},
H. Feng$^{1}$,
L. Feng$^{14}$,
S.H. Feng$^{1,3}$,
X.T. Feng$^{22}$,
Y. Feng$^{15}$,
Y.L. Feng$^{18}$,
S. Gabici$^{23}$,
B. Gao$^{1,3}$,
C.D. Gao$^{22}$,
Q. Gao$^{18}$,
W. Gao$^{1,3}$,
W.K. Gao$^{1,2,3}$,
M.M. Ge$^{17}$,
T.T. Ge$^{21}$,
L.S. Geng$^{1,3}$,
G. Giacinti$^{9}$,
G.H. Gong$^{24}$,
Q.B. Gou$^{1,3}$,
M.H. Gu$^{1,3,13}$,
F.L. Guo$^{16}$,
J. Guo$^{24}$,
X.L. Guo$^{6}$,
Y.Q. Guo$^{1,3}$,
Y.Y. Guo$^{14}$,
Y.A. Han$^{25}$,
O.A. Hannuksela$^{19}$,
M. Hasan$^{1,2,3}$,
H.H. He$^{1,2,3}$,
H.N. He$^{14}$,
J.Y. He$^{14}$,
Y. He$^{6}$,
Y.K. Hor$^{21}$,
B.W. Hou$^{1,2,3}$,
C. Hou$^{1,3}$,
H.B. Hu$^{1,2,3}$,
Q. Hu$^{12,14}$,
S.C. Hu$^{1,3,27}$,
C. Huang$^{7}$,
D.H. Huang$^{6}$,
T.Q. Huang$^{1,3}$,
W.J. Huang$^{21}$,
X.T. Huang$^{22}$,
X.Y. Huang$^{14}$,
Y. Huang$^{1,2,3}$,
Y.Y. Huang$^{7}$,
X.L. Ji$^{1,3,13}$,
H.Y. Jia$^{6}$,
K. Jia$^{22}$,
H.B. Jiang$^{1,3}$,
K. Jiang$^{13,12}$,
X.W. Jiang$^{1,3}$,
Z.J. Jiang$^{17}$,
M. Jin$^{6}$,
M.M. Kang$^{28}$,
I. Karpikov$^{10}$,
D. Khangulyan$^{1,3}$,
D. Kuleshov$^{10}$,
K. Kurinov$^{10}$,
B.B. Li$^{11}$,
C.M. Li$^{7}$,
Cheng Li$^{13,12}$,
Cong Li$^{1,3}$,
D. Li$^{1,2,3}$,
F. Li$^{1,3,13}$,
H.B. Li$^{1,3}$,
H.C. Li$^{1,3}$,
Jian Li$^{12}$,
Jie Li$^{1,3,13}$,
K. Li$^{1,3}$,
S.D. Li$^{16,2}$,
W.L. Li$^{22}$,
W.L. Li$^{9}$,
X.R. Li$^{1,3}$,
Xin Li$^{13,12}$,
Y.Z. Li$^{1,2,3}$,
Zhe Li$^{1,3}$,
Zhuo Li$^{29}$,
E.W. Liang$^{30}$,
Y.F. Liang$^{30}$,
S.J. Lin$^{21}$,
B. Liu$^{12}$,
C. Liu$^{1,3}$,
D. Liu$^{22}$,
D.B. Liu$^{9}$,
H. Liu$^{6}$,
H.D. Liu$^{25}$,
J. Liu$^{1,3}$,
J.L. Liu$^{1,3}$,
M.Y. Liu$^{18}$,
R.Y. Liu$^{7}$,
S.M. Liu$^{6}$,
W. Liu$^{1,3}$,
Y. Liu$^{8}$,
Y.N. Liu$^{24}$,
Q. Luo$^{21}$,
Y. Luo$^{9}$,
H.K. Lv$^{1,3}$,
B.Q. Ma$^{29}$,
L.L. Ma$^{1,3}$,
X.H. Ma$^{1,3}$,
J.R. Mao$^{26}$\thanks{\href{mailto:jirongmao@mail.ynao.ac.cn}{jirongmao@mail.ynao.ac.cn}}，
Z. Min$^{1,3}$,
W. Mitthumsiri$^{31}$,
H.J. Mu$^{25}$,
Y.C. Nan$^{1,3}$,
A. Neronov$^{23}$,
K.C.Y. Ng$^{19}$,
L.J. Ou$^{8}$,
P. Pattarakijwanich$^{31}$,
Z.Y. Pei$^{8}$,
J.C. Qi$^{1,2,3}$,
M.Y. Qi$^{1,3}$,
B.Q. Qiao$^{1,3}$,
J.J. Qin$^{12}$,
A. Raza$^{1,2,3}$,
D. Ruffolo$^{31}$,
A. S\'aiz$^{31}$,
M. Saeed$^{1,2,3}$,
D. Semikoz$^{23}$,
L. Shao$^{11}$,
O. Shchegolev$^{10,32}$,
X.D. Sheng$^{1,3}$,
F.W. Shu$^{33}$,
H.C. Song$^{29}$,
Yu.V. Stenkin$^{10,32}$,
V. Stepanov$^{10}$,
Y. Su$^{14}$,
D.X. Sun$^{12,14}$,
Q.N. Sun$^{6}$,
X.N. Sun$^{30}$,
Z.B. Sun$^{34}$,
J. Takata$^{35}$,
P.H.T. Tam$^{21}$,
Q.W. Tang$^{33}$,
R. Tang$^{9}$,
Z.B. Tang$^{13,12}$,
W.W. Tian$^{2,20}$,
L.H. Wan$^{21}$,
C. Wang$^{34}$,
C.B. Wang$^{6}$,
G.W. Wang$^{12}$,
H.G. Wang$^{8}$,
H.H. Wang$^{21}$,
J.C. Wang$^{26}$,
Kai Wang$^{7}$,
Kai Wang$^{35}$,
L.P. Wang$^{1,2,3}$,
L.Y. Wang$^{1,3}$,
P.H. Wang$^{6}$,
R. Wang$^{22}$\thanks{\href{mailto:ranw@mail.sdu.edu.cn}{ranw@mail.sdu.edu.cn}},
W. Wang$^{21}$,
X.G. Wang$^{30}$,
X.Y. Wang$^{7}$,
Y. Wang$^{6}$,
Y.D. Wang$^{1,3}$,
Y.J. Wang$^{1,3}$,
Z.H. Wang$^{28}$,
Z.X. Wang$^{17}$,
Zhen Wang$^{9}$,
Zheng Wang$^{1,3,13}$,
D.M. Wei$^{14}$,
J.J. Wei$^{14}$,
Y.J. Wei$^{1,2,3}$,
T. Wen$^{17}$,
C.Y. Wu$^{1,3}$,
H.R. Wu$^{1,3}$,
Q.W. Wu$^{35}$,
S. Wu$^{1,3}$,
X.F. Wu$^{14}$,
Y.S. Wu$^{12}$,
S.Q. Xi$^{1,3}$,
J. Xia$^{12,14}$,
G.M. Xiang$^{16,2}$,
D.X. Xiao$^{11}$,
G. Xiao$^{1,3}$,
Y.L. Xin$^{6}$,
Y. Xing$^{16}$,
D.R. Xiong$^{26}$,
Z. Xiong$^{1,2,3}$,
D.L. Xu$^{9}$,
R.F. Xu$^{1,2,3}$,
R.X. Xu$^{29}$,
W.L. Xu$^{28}$,
L. Xue$^{22}$,
D.H. Yan$^{17}$,
J.Z. Yan$^{14}$,
T. Yan$^{1,3}$,
C.W. Yang$^{28}$,
C.Y. Yang$^{26}$\thanks{\href{mailto:chyyo@ynao.ac.cn}{chyy@ynao.ac.cn}},
F. Yang$^{11}$,
F.F. Yang$^{1,3,13}$,
L.L. Yang$^{21}$,
M.J. Yang$^{1,3}$,
R.Z. Yang$^{12}$,
W.X. Yang$^{8}$,
Y.H. Yao$^{1,3}$,
Z.G. Yao$^{1,3}$,
L.Q. Yin$^{1,3}$,
N. Yin$^{22}$,
X.H. You$^{1,3}$,
Z.Y. You$^{1,3}$,
Y.H. Yu$^{12}$,
Q. Yuan$^{14}$,
H. Yue$^{1,2,3}$,
H.D. Zeng$^{14}$,
T.X. Zeng$^{1,3,13}$,
W. Zeng$^{17}$,
M. Zha$^{1,3}$\thanks{\href{mailto:zham@ihep.ac.cn}{zham@ihep.ac.cn}},
B.B. Zhang$^{7}$,
F. Zhang$^{6}$,
H. Zhang$^{9}$,
H.M. Zhang$^{7}$,
H.Y. Zhang$^{17}$,
J.L. Zhang$^{20}$,
Li Zhang$^{17}$,
P.F. Zhang$^{17}$,
P.P. Zhang$^{12,14}$,
R. Zhang$^{14}$,
S.B. Zhang$^{2,20}$,
S.R. Zhang$^{11}$,
S.S. Zhang$^{1,3}$,
X. Zhang$^{7}$,
X.P. Zhang$^{1,3}$,
Y.F. Zhang$^{6}$,
Yi Zhang$^{1,14}$,
Yong Zhang$^{1,3}$,
B. Zhao$^{6}$,
J. Zhao$^{1,3}$,
L. Zhao$^{13,12}$,
L.Z. Zhao$^{11}$,
S.P. Zhao$^{14}$,
X.H. Zhao$^{26}$,
F. Zheng$^{34}$,
W.J. Zhong$^{7}$,
B. Zhou$^{1,3}$,
H. Zhou$^{9}$,
J.N. Zhou$^{16}$,
M. Zhou$^{33}$,
P. Zhou$^{7}$,
R. Zhou$^{28}$,
X.X. Zhou$^{1,2,3}$,
X.X. Zhou$^{6}$,
B.Y. Zhu$^{12,14}$,
C.G. Zhu$^{22}$,
F.R. Zhu$^{6}$,
H. Zhu$^{20}$,
K.J. Zhu$^{1,2,3,13}$,
Y.C. Zou$^{35}$,
X. Zuo$^{1,3}$,(LHAASO Collaboration)
}
%\newauthor (Affiliations can be found after the references)
}



==> Science20240601.tex <==
Zhen Cao$^{1,2,3}$,
F. Aharonian$^{4,5}$,
Axikegu$^{6}$,
Y.X. Bai$^{1,3}$,
Y.W. Bao$^{7}$,
D. Bastieri$^{8}$,
X.J. Bi$^{1,2,3}$,
Y.J. Bi$^{1,3}$,
W. Bian$^{9}$,
A.V. Bukevich$^{10}$,
Q. Cao$^{11}$,
W.Y. Cao$^{12}$,
Zhe Cao$^{13,12}$,
J. Chang$^{14}$,
J.F. Chang$^{1,3,13}$,
A.M. Chen$^{9}$,
E.S. Chen$^{1,2,3}$,
H.X. Chen$^{15}$,
Liang Chen$^{16}$,
Lin Chen$^{6}$,
Long Chen$^{6}$,
M.J. Chen$^{1,3}$,
M.L. Chen$^{1,3,13}$,
Q.H. Chen$^{6}$,
S. Chen$^{17}$,
S.H. Chen$^{1,2,3}$,
S.Z. Chen$^{1,3}$,
T.L. Chen$^{18}$,
Y. Chen$^{7}$,
N. Cheng$^{1,3}$,
Y.D. Cheng$^{1,2,3}$,
M.C. Chu$^{19}$,
M.Y. Cui$^{14}$,
S.W. Cui$^{11}$,
X.H. Cui$^{20}$,
Y.D. Cui$^{21}$,
B.Z. Dai$^{17}$,
H.L. Dai$^{1,3,13}$,
Z.G. Dai$^{12}$,
Danzengluobu$^{18}$,
X.Q. Dong$^{1,2,3}$,
K.K. Duan$^{14}$,
J.H. Fan$^{8}$,
Y.Z. Fan$^{14}$,
J. Fang$^{17}$,
J.H. Fang$^{15}$,
K. Fang$^{1,3}$,
C.F. Feng$^{22}$,
H. Feng$^{1}$,
L. Feng$^{14}$,
S.H. Feng$^{1,3}$,
X.T. Feng$^{22}$,
Y. Feng$^{15}$,
Y.L. Feng$^{18}$,
S. Gabici$^{23}$,
B. Gao$^{1,3}$,
C.D. Gao$^{22}$,
Q. Gao$^{18}$,
W. Gao$^{1,3}$,
W.K. Gao$^{1,2,3}$,
M.M. Ge$^{17}$,
T.T. Ge$^{21}$,
L.S. Geng$^{1,3}$,
G. Giacinti$^{9}$,
G.H. Gong$^{24}$,
Q.B. Gou$^{1,3}$,
M.H. Gu$^{1,3,13}$,
F.L. Guo$^{16}$,
J. Guo$^{24}$,
X.L. Guo$^{6}$,
Y.Q. Guo$^{1,3}$,
Y.Y. Guo$^{14}$,
Y.A. Han$^{25}$,
O.A. Hannuksela$^{19}$,
M. Hasan$^{1,2,3}$,
H.H. He$^{1,2,3}$,
H.N. He$^{14}$,
J.Y. He$^{14}$,
Y. He$^{6}$,
Y.K. Hor$^{21}$,
B.W. Hou$^{1,2,3}$,
C. Hou$^{1,3}$,
X. Hou$^{26}$,
H.B. Hu$^{1,2,3}$,
Q. Hu$^{12,14}$,
S.C. Hu$^{1,3,27}$,
C. Huang$^{7}$,
D.H. Huang$^{6}$,
T.Q. Huang$^{1,3}$,
W.J. Huang$^{21}$,
X.T. Huang$^{22}$,
X.Y. Huang$^{14}$,
Y. Huang$^{1,2,3}$,
Y.Y. Huang$^{7}$,
X.L. Ji$^{1,3,13}$,
H.Y. Jia$^{6}$,
K. Jia$^{22}$,
H.B. Jiang$^{1,3}$,
K. Jiang$^{13,12}$,
X.W. Jiang$^{1,3}$,
Z.J. Jiang$^{17}$,
M. Jin$^{6}$,
M.M. Kang$^{28}$,
I. Karpikov$^{10}$,
D. Khangulyan$^{1,3}$,
D. Kuleshov$^{10}$,
K. Kurinov$^{10}$,
B.B. Li$^{11}$,
C.M. Li$^{7}$,
Cheng Li$^{13,12}$,
Cong Li$^{1,3}$,
D. Li$^{1,2,3}$,
F. Li$^{1,3,13}$,
H.B. Li$^{1,3}$,
H.C. Li$^{1,3}$,
Jian Li$^{12}$,
Jie Li$^{1,3,13}$,
K. Li$^{1,3}$,
S.D. Li$^{16,2}$,
W.L. Li$^{22}$,
W.L. Li$^{9}$,
X.R. Li$^{1,3}$,
Xin Li$^{13,12}$,
Y.Z. Li$^{1,2,3}$,
Zhe Li$^{1,3}$,
Zhuo Li$^{29}$,
E.W. Liang$^{30}$,
Y.F. Liang$^{30}$,
S.J. Lin$^{21}$,
B. Liu$^{12}$,
C. Liu$^{1,3}$,
D. Liu$^{22}$,
D.B. Liu$^{9}$,
H. Liu$^{6}$,
H.D. Liu$^{25}$,
J. Liu$^{1,3}$,
J.L. Liu$^{1,3}$,
M.Y. Liu$^{18}$,
R.Y. Liu$^{7}$,
S.M. Liu$^{6}$,
W. Liu$^{1,3}$,
Y. Liu$^{8}$,
Y.N. Liu$^{24}$,
Q. Luo$^{21}$,
Y. Luo$^{9}$,
H.K. Lv$^{1,3}$,
B.Q. Ma$^{29}$,
L.L. Ma$^{1,3}$,
X.H. Ma$^{1,3}$,
J.R. Mao$^{26}$,
Z. Min$^{1,3}$,
W. Mitthumsiri$^{31}$,
H.J. Mu$^{25}$,
Y.C. Nan$^{1,3}$,
A. Neronov$^{23}$,
K.C.Y. Ng$^{19}$,
L.J. Ou$^{8}$,
P. Pattarakijwanich$^{31}$,
Z.Y. Pei$^{8}$,
J.C. Qi$^{1,2,3}$,
M.Y. Qi$^{1,3}$,
B.Q. Qiao$^{1,3}$,
J.J. Qin$^{12}$,
A. Raza$^{1,2,3}$,
D. Ruffolo$^{31}$,
A. S\'aiz$^{31}$,
M. Saeed$^{1,2,3}$,
D. Semikoz$^{23}$,
L. Shao$^{11}$,
O. Shchegolev$^{10,32}$,
X.D. Sheng$^{1,3}$,
F.W. Shu$^{33}$,
H.C. Song$^{29}$,
Yu.V. Stenkin$^{10,32}$,
V. Stepanov$^{10}$,
Y. Su$^{14}$,
D.X. Sun$^{12,14}$,
Q.N. Sun$^{6}$,
X.N. Sun$^{30}$,
Z.B. Sun$^{34}$,
J. Takata$^{35}$,
P.H.T. Tam$^{21}$,
Q.W. Tang$^{33}$,
R. Tang$^{9}$,
Z.B. Tang$^{13,12}$,
W.W. Tian$^{2,20}$,
L.H. Wan$^{21}$,
C. Wang$^{34}$,
C.B. Wang$^{6}$,
G.W. Wang$^{12}$,
H.G. Wang$^{8}$,
H.H. Wang$^{21}$,
J.C. Wang$^{26}$,
Kai Wang$^{7}$,
Kai Wang$^{35}$,
L.P. Wang$^{1,2,3}$,
L.Y. Wang$^{1,3}$,
P.H. Wang$^{6}$,
R. Wang$^{22}$,
W. Wang$^{21}$,
X.G. Wang$^{30}$,
X.Y. Wang$^{7}$,
Y. Wang$^{6}$,
Y.D. Wang$^{1,3}$,
Y.J. Wang$^{1,3}$,
Z.H. Wang$^{28}$,
Z.X. Wang$^{17}$,
Zhen Wang$^{9}$,
Zheng Wang$^{1,3,13}$,
D.M. Wei$^{14}$,
J.J. Wei$^{14}$,
Y.J. Wei$^{1,2,3}$,
T. Wen$^{17}$,
C.Y. Wu$^{1,3}$,
H.R. Wu$^{1,3}$,
Q.W. Wu$^{35}$,
S. Wu$^{1,3}$,
X.F. Wu$^{14}$,
Y.S. Wu$^{12}$,
S.Q. Xi$^{1,3}$,
J. Xia$^{12,14}$,
G.M. Xiang$^{16,2}$,
D.X. Xiao$^{11}$,
G. Xiao$^{1,3}$,
Y.L. Xin$^{6}$,
Y. Xing$^{16}$,
D.R. Xiong$^{26}$,
Z. Xiong$^{1,2,3}$,
D.L. Xu$^{9}$,
R.F. Xu$^{1,2,3}$,
R.X. Xu$^{29}$,
W.L. Xu$^{28}$,
L. Xue$^{22}$,
D.H. Yan$^{17}$,
J.Z. Yan$^{14}$,
T. Yan$^{1,3}$,
C.W. Yang$^{28}$,
C.Y. Yang$^{26}$,
F. Yang$^{11}$,
F.F. Yang$^{1,3,13}$,
L.L. Yang$^{21}$,
M.J. Yang$^{1,3}$,
R.Z. Yang$^{12}$,
W.X. Yang$^{8}$,
Y.H. Yao$^{1,3}$,
Z.G. Yao$^{1,3}$,
L.Q. Yin$^{1,3}$,
N. Yin$^{22}$,
X.H. You$^{1,3}$,
Z.Y. You$^{1,3}$,
Y.H. Yu$^{12}$,
Q. Yuan$^{14}$,
H. Yue$^{1,2,3}$,
H.D. Zeng$^{14}$,
T.X. Zeng$^{1,3,13}$,
W. Zeng$^{17}$,
M. Zha$^{1,3}$,
B.B. Zhang$^{7}$,
F. Zhang$^{6}$,
H. Zhang$^{9}$,
H.M. Zhang$^{7}$,
H.Y. Zhang$^{17}$,
J.L. Zhang$^{20}$,
Li Zhang$^{17}$,
P.F. Zhang$^{17}$,
P.P. Zhang$^{12,14}$,
R. Zhang$^{14}$,
S.B. Zhang$^{2,20}$,
S.R. Zhang$^{11}$,
S.S. Zhang$^{1,3}$,
X. Zhang$^{7}$,
X.P. Zhang$^{1,3}$,
Y.F. Zhang$^{6}$,
Yi Zhang$^{1,14}$,
Yong Zhang$^{1,3}$,
B. Zhao$^{6}$,
J. Zhao$^{1,3}$,
L. Zhao$^{13,12}$,
L.Z. Zhao$^{11}$,
S.P. Zhao$^{14}$,
X.H. Zhao$^{26}$,
F. Zheng$^{34}$,
W.J. Zhong$^{7}$,
B. Zhou$^{1,3}$,
H. Zhou$^{9}$,
J.N. Zhou$^{16}$,
M. Zhou$^{33}$,
P. Zhou$^{7}$,
R. Zhou$^{28}$,
X.X. Zhou$^{1,2,3}$,
X.X. Zhou$^{6}$,
B.Y. Zhu$^{12,14}$,
C.G. Zhu$^{22}$,
F.R. Zhu$^{6}$,
H. Zhu$^{20}$,
K.J. Zhu$^{1,2,3,13}$,
Y.C. Zou$^{35}$,
X. Zuo$^{1,3}$,
(The LHAASO Collaboration)
$^{1}$ Key Laboratory of Particle Astrophysics \& Experimental Physics Division \& Computing Center, Institute of High Energy Physics, Chinese Academy of Sciences, 100049 Beijing, China\\
$^{2}$ University of Chinese Academy of Sciences, 100049 Beijing, China\\
$^{3}$ TIANFU Cosmic Ray Research Center, Chengdu, Sichuan,  China\\
$^{4}$ Dublin Institute for Advanced Studies, 31 Fitzwilliam Place, 2 Dublin, Ireland \\
$^{5}$ Max-Planck-Institut for Nuclear Physics, P.O. Box 103980, 69029  Heidelberg, Germany\\
$^{6}$ School of Physical Science and Technology \&  School of Information Science and Technology, Southwest Jiaotong University, 610031 Chengdu, Sichuan, China\\
$^{7}$ School of Astronomy and Space Science, Nanjing University, 210023 Nanjing, Jiangsu, China\\
$^{8}$ Center for Astrophysics, Guangzhou University, 510006 Guangzhou, Guangdong, China\\
$^{9}$ Tsung-Dao Lee Institute \& School of Physics and Astronomy, Shanghai Jiao Tong University, 200240 Shanghai, China\\
$^{10}$ Institute for Nuclear Research of Russian Academy of Sciences, 117312 Moscow, Russia\\
$^{11}$ Hebei Normal University, 050024 Shijiazhuang, Hebei, China\\
$^{12}$ University of Science and Technology of China, 230026 Hefei, Anhui, China\\
$^{13}$ State Key Laboratory of Particle Detection and Electronics, China\\
$^{14}$ Key Laboratory of Dark Matter and Space Astronomy \& Key Laboratory of Radio Astronomy, Purple Mountain Observatory, Chinese Academy of Sciences, 210023 Nanjing, Jiangsu, China\\
$^{15}$ Research Center for Astronomical Computing, Zhejiang Laboratory, 311121 Hangzhou, Zhejiang, China\\
$^{16}$ Key Laboratory for Research in Galaxies and Cosmology, Shanghai Astronomical Observatory, Chinese Academy of Sciences, 200030 Shanghai, China\\
$^{17}$ School of Physics and Astronomy, Yunnan University, 650091 Kunming, Yunnan, China\\
$^{18}$ Key Laboratory of Cosmic Rays (Tibet University), Ministry of Education, 850000 Lhasa, Tibet, China\\
$^{19}$ Department of Physics, The Chinese University of Hong Kong, Shatin, New Territories, Hong Kong, China\\
$^{20}$ Key Laboratory of Radio Astronomy and Technology, National Astronomical Observatories, Chinese Academy of Sciences, 100101 Beijing, China\\
$^{21}$ School of Physics and Astronomy (Zhuhai) \& School of Physics (Guangzhou) \& Sino-French Institute of Nuclear Engineering and Technology (Zhuhai), Sun Yat-sen University, 519000 Zhuhai \& 510275 Guangzhou, Guangdong, China\\
$^{22}$ Institute of Frontier and Interdisciplinary Science, Shandong University, 266237 Qingdao, Shandong, China\\
$^{23}$ APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, CEA/IRFU, Observatoire de Paris, 119 75205 Paris, France\\
$^{24}$ Department of Engineering Physics \& Department of Astronomy, Tsinghua University, 100084 Beijing, China\\
$^{25}$ School of Physics and Microelectronics, Zhengzhou University, 450001 Zhengzhou, Henan, China\\
$^{26}$ Yunnan Observatories, Chinese Academy of Sciences, 650216 Kunming, Yunnan, China\\
$^{27}$ China Center of Advanced Science and Technology, Beijing 100190, China\\
$^{28}$ College of Physics, Sichuan University, 610065 Chengdu, Sichuan, China\\
$^{29}$ School of Physics, Peking University, 100871 Beijing, China\\
$^{30}$ Guangxi Key Laboratory for Relativistic Astrophysics, School of Physical Science and Technology, Guangxi University, 530004 Nanning, Guangxi, China\\
$^{31}$ Department of Physics, Faculty of Science, Mahidol University, Bangkok 10400, Thailand\\
$^{32}$ Moscow Institute of Physics and Technology, 141700 Moscow, Russia\\
$^{33}$ Center for Relativistic Astrophysics and High Energy Physics, School of Physics and Materials Science \& Institute of Space Science and Technology, Nanchang University, 330031 Nanchang, Jiangxi, China\\
$^{34}$ National Space Science Center, Chinese Academy of Sciences, 100190 Beijing, China\\
$^{35}$ School of Physics, Huazhong University of Science and Technology, Wuhan 430074, Hubei, China\\

